Do Prompts Solve NLP Tasks Using Natural Language?

Thanks to the advanced improvement of large pre-trained language models, prompt-based fine-tuning is shown to be effective on a variety of downstream tasks. Though many prompting methods have been investigated, it remains unknown which type of prompts are the most effective among three types of prompts (i.e., human-designed prompts, schema prompts and null prompts). In this work, we empirically compare the three types of prompts under both few-shot and fully-supervised settings. Our experimental results show that schema prompts are the most effective in general. Besides, the performance gaps tend to diminish when the scale of training data grows large.

==> sections/introduction_old.tex <==
\section{Introduction}
Thanks to the advanced improvement of large pre-trained language models~\cite{devlin-etal-2019-bert,liu2019roberta,gpt-3}, prompt-based fine-tuning is shown to be effective on a variety of downstream tasks~\cite{shin-etal-2020-autoprompt,schick-etal-2020-automatically,tanl}, under both few-shot and fully-supervised settings. 
% such as sentiment classification~\cite{shin-etal-2020-autoprompt,schick-etal-2020-automatically,gao2021making}, named entity recognition~\cite{cui-etal-2021-template,tanl} and dialogue state tracking~\cite{lee2021dialogue}, under both few-shot and fully-supervised settings. 
% These methods can be generally divided into two folds according to their prompt types: cloze-style prompt using masked language models and prefix-based prompt using autoregressive language models. 
% In particular, they are demonstrated to be efficient few-shot learners~\cite{brown2020language,gao2021making}, consistently outperforming traditional fine-tuning methods when the number of labeled instances is limited. 
Given an input, prompt-based fine-tuning adopts the language modeling head to generate meaningful words based on prompts instead of hollow classification label indices; thus, rich meanings in pre-trained dense word representations get exploited. 

It is intuitive that a good prompt should be a fluent sentence that contains task-specific hints, 
% which describe the task, prompt用可以描述任务的自然语言，到底什么样的prompt起到提示作用
% just the way in which humans develop their languages and in which language models are pretrained \cite{}. 
just the way in which previous work probe factual knowledge from pretrained language models~\cite{petroni-etal-2019-language,jiang-etal-2020-know}.
Following this line, previous work explored a variety of {\it template}-based prompts to solve down-stream tasks~\cite{schick-schutze-2021-just,gao2021making,cui-etal-2021-template}. 
% However, another line of work that adopts schema-based prompts also achieved impressive performance, showing that it might be unnecessary for prompts to follow human speaking or writing~\cite{feng-etal-2021-sequence,tanl,lee2021dialogue}. 
% % For example, if a input for sentiment analysis is ``{\it THIS MOVIE IS AMAZING!!!}'' a template might be ``{\it <Input> \underline{This movie was {\tt [MASK]}}}'', while a schema could be ``{\it <Input> \underline{Sentiment: {\tt [MASK]}}}''. 
However, other work suggested that syntactically-incorrect prompts (e.g., automatically searched prompts~\cite{shin-etal-2020-autoprompt,gao2021making} and {\it schema}-based prompts~\cite{lee2021dialogue}) and task-agnostic prompts~\cite{logan2021cutting} might also work well.
% As shown in Table~\ref{tab:prompt_examples}, schema-based prompts make pure use of rich semantics in pretrained word representations and discard most syntactic traits, yet still work well. 
Table~\ref{tab:intro_example} shows an example.
% In this way, they get rid of complicated template-design and thus allow more flexible transfer among different domains or tasks~\cite{tanl}. 

\input{table_and_figure/intro_example}

Tracking this interesting yet counter-intuitive result, we would like to know: {\it What aspects of prompts empower prompt-based fine-tuning? }
% Though much work on prompt-based fine-tuning has been done, our question remains unexplored. 
% Recently, ~\citet{logan2021cutting} partially addressed our question by proposing to use a task-agnostic prompt (i.e., {\it null} prompt) instead of human-like prompt for few-shot fine-tuning, but their exploration is somehow limited: they only compare existing human-like prompt with {\it null} prompt. 
%
% To this end, we ask three questions about prompt properties of prompt-based fine-tuning and conduct a systematic analysis:
In particular, we ask three questions about prompt properties of prompt-based fine-tuning and conduct a systematic analysis:

First, {\it do prompts have to follow human speaking and writing?} 
We might expect human-spoken prompt (i.e., template-based prompt) to outperform schema-based prompt, because prompting methods are based on pretrained language models whose pretrained corpora are human spoken and written texts. 
From our experiments, we find that {\bf prompts do not necessarily need to be grammatically-correct sentences}. 
Instead, schema-based prompts achieve the best overall performance for both sentence classification and structure prediction tasks under few-shot settings.

Second, {\it do prompts have to contain task-specific hints,} or are task-agnostic {\it null} prompts competitive enough to do the job?
\citet{logan2021cutting} empirically showed that {\it\ null} prompts achieved competitive performance on several sentence-pair and passage-sentence classification tasks, but our results indicate that {\bf task-agnostic prompts (i.e., \textbf{\textit{null}} prompts) are mostly worse than task-specific prompts under the few-shot setting}.
In particular, {\it null} prompts underperform schema-based prompts for seven out of eight single-sentence classification tasks in our experiments.

Finally, putting aside the impact of prompt patterns, {\it how do label word choices influence prompting methods?}
% Previous work explored automatic label word search, which adopts a vanilla pretrained language model to find the top-$k$ label tokens~\cite{gao2021making}.
We find that the choices of label tokens are not strictly constrained to some particular words, but {\bf automatically searched loosely-connected synonyms could do the job}.
Besides, our results suggest that initializing the label words with pretrained token embeddings is extremely helpful for few-shot settings, which is in line with previous work~\cite{li-liang-2021-prefix,lester-etal-2021-power}.
%这个跟prefix tuning没什么关系吧, 突出few shot 有prompt pattern效果更好

%任务分类是不是按sentence和token分比较好
% intro + we conduct our experiments on both sentence-level tasks and token-levels tasks

% In particular, we seek to find out: (1) whether or not schema-based prompts' competitive performance could generalize well to a variety of tasks, and why; (2) how different prompts perform under different settings (i.e., few-shot and fully-supervised settings).
% Besides, since schema-based prompts largely reduce the efforts of prompt design, more attention could be paid to another part of prompt engineering, label word. 
% To find out the impact of label word, in addition to traditional hand-crafted label tokens, we also experiment with automatically-searched label words~\cite{gao2021making} and randomly-initialized placeholders.
% Our analysis is under both few-shot and fully-supervised settings, using a single prompt for each task as well as multi-prompt ensemble. 




% Based on our experiments, we find that:
% \begin{itemize}
%     \item Structure prediction and sentence classification tasks exhibit different xxxxxxxxx when using xxxxx
%     \item zzz
% \end{itemize}


% sentiment analysis: sst-2, sst-5, MR movie reviews, CR
% Subjectivity: Subj
% Text REtrieval Conference (TREC) Question Classification
% The Corpus of Linguistic Acceptability (CoLA)

% \section{Related Work}
% Recent trend on prompt-tuning was mainly motivated by the success of GPT models~\cite{gpt-1,gpt-2,gpt-3}.

==> table_and_figure/number_of_wins.tex <==
\begin{table}[h!]
    \centering
    % \fontsize{11}{12}\selectfont
    % \resizebox{0.96\textwidth}{!}{
    \begin{adjustbox}{max width=0.48\textwidth}
    \begin{tabular}{lccc}
        \hline
        \multirow{2}{*}{\bf Method}  & \multicolumn{3}{c}{\bf \# Wins} \\
        %   & {\bf Few}  & {\bf Full} & {\bf Both} \\
          & {Few}  & {Full} & {Total} \\
        \hline
         Fine-tuning                       & 1 & 1 & 2 \\
        %  LM-BFF~$\dagger$                  &  &  &  \\
         Template Prompt                   & 0 & 0 & 0 \\
         \hspace{0.5em} w/ auto label word & 0 & 1 & 1 \\
         \hspace{0.5em} w/ special token   & 0 & 1 & 1 \\
         Schema Prompt                     & 1 & 1 & 2 \\
         \hspace{0.5em} w/ auto label word & {\bf 5} & 1 & {\bf 6} \\
         \hspace{0.5em} w/ special token   & 1 & {\bf 3} & 4 \\
         {\it Null} Prompt                 & 0 & 1 & 1 \\
        \hline
    \end{tabular}
    \end{adjustbox}
    % }
    \caption{Number of wins of the performance using different types of prompts. }
    \label{tab:num_wins}
    % \vspace{-10pt}
\end{table}

==> table_and_figure/results_full.tex <==
% \begin{table*}[h!]
%     \centering
%     % \fontsize{11}{12}\selectfont
%     % \resizebox{0.96\textwidth}{!}{
%     \begin{adjustbox}{max width=\textwidth}
%     \begin{tabular}{lcccccccc}
%         \hline
%           & \textbf{SST-2} & \textbf{SST-5} & \textbf{MR} & \textbf{CR} & \textbf{MPQA} & \textbf{Subj} & \textbf{TREC} & \textbf{CoLA}\\
%           & (acc) & (acc) & (acc) & (acc) & (acc) & (acc) & (acc) & (Matt.) \\
%         %  & \multicolumn{2}{c}{(Acc)} & \multicolumn{2}{c}{(Acc)} & \multicolumn{2}{c}{(Acc)} & \multicolumn{2}{c}{(Acc)} \\
%         %   & Few  & Full  & Few & Full  &  Few & Full &  Few & Full \\
%         \hline
%          Fine-tuning                       & 95.0 & 58.7 & 90.8 & 89.4 & 87.8 & {\bf 97.0} & 97.4 & 62.6 \\ 
%         %  LM-BFF~$\dagger$                  & 93.0 (0.6)        & --         & 49.5 (1.7)  & --   & {\bf 87.7 (1.4)} & --   & 91.0 (0.9) & -- \\ 
%         \cline{1-9} 
%          Template Prompt                   & 95.1 & 59.0 & 91.2 & 91.6 & 89.8 & 95.5 & 96.8 & 66.3 \\ 
%          \hspace{0.5em} w/ auto label word & 95.6 & 58.8 & 91.7 & 91.3 & 90.8 & 95.8 & 97.0 & {\bf 68.0} \\ 
%          \hspace{0.5em} w/ special token   & 95.6 & 58.3 & 91.6 & {\bf 92.7} & 90.3 & 96.4 & 84.8 & 65.4 \\ 
%          Schema Prompt                     & 95.2 & {\bf 59.4} & 91.4 & 91.8 & 90.2 & 95.6 & 97.2 & 67.0 \\ 
%          \hspace{0.5em} w/ auto label word & 95.1 & 58.4 & 91.9 & 91.9 & 89.8 & 96.7 & {\bf 97.6} & 66.4 \\ 
%          \hspace{0.5em} w/ special token   & {\bf 95.8} & 57.7 & {\bf 92.4} & 91.4 & {\bf 90.9} & 96.4 & 97.2 & 67.8 \\ 
%          {\it Null} Prompt                 & 95.7 & 55.9 & 90.5 & 87.5 & 90.8 & 96.0 & 96.4 & {\bf 68.0} \\ 
%         \hline
%     \end{tabular}
%     \end{adjustbox}
%     % }
%     \caption{Full-size experiment results. 
%             % $\dagger$ means that we report the automatic template setting of LM-BFF~\cite{gao2021making}, which obtained the best overall results in their paper. 
%             The results with {\it null} prompt~\cite{logan2021cutting} are produced by our re-implementation. 
%             The results with {\it null} prompts should be compared with template- and schema-based prompts without auto label word or special token. }
%     % \label{tab:results_full}
%     % \vspace{-10pt}
% \end{table*}
